Multi-transversals for Triangles and the Tuza's Conjecture

In this paper, we study a primal and dual relationship about triangles: For any graph $G$, let $\nu(G)$ be the maximum number of edge-disjoint triangles in $G$, and $\tau(G)$ be the minimum subset $F$ of edges such that $G \setminus F$ is triangle-free. It is easy to see that $\nu(G) \leq \tau(G) \leq 3 \nu(G)$, and in fact, this rather obvious inequality holds for a much more general primal-dual relation between $k$-hyper matching and covering in hypergraphs. Tuza conjectured in $1981$ that $\tau(G) \leq 2 \nu(G)$, and this question has received attention from various groups of researchers in discrete mathematics, settling various special cases such as planar graphs and generalized to bounded maximum average degree graphs, some cases of minor-free graphs, and very dense graphs. Despite these efforts, the conjecture in general graphs has remained wide open for almost four decades. In this paper, we provide a proof of a non-trivial consequence of the conjecture; that is, for every $k \geq 2$, there exist a (multi)-set $F \subseteq E(G): |F| \leq 2k \nu(G)$ such that each triangle in $G$ overlaps at least $k$ elements in $F$. Our result can be seen as a strengthened statement of Krivelevich's result on the fractional version of Tuza's conjecture (and we give some examples illustrating this.) The main technical ingredient of our result is a charging argument, that locally identifies edges in $F$ based on a local view of the packing solution. This idea might be useful in further studying the primal-dual relations in general and the Tuza's conjecture in particular.

==> tex/half-int.tex <==
\section{Multi-transversals of order two}
\label{sec:order-2}

Again, this is equivalence to finding the assignment $f: E \rightarrow {\mathbb R}^+$ such that $f(e) \in \{\frac j {2}: j \in \{0, 1, 2\}\}$ where $\sum_e f(e) \leq 2 |\Nu|$ and for all $t \in \tset$, $\sum_{e \in E(t)} f(e) \geq 1$.

This section will go in the following order. First we will describe an initial distribution scheme and then a re-distribution scheme based on two key structural lemmas and show how to use them to get the result. Finally, we will prove these two lemmas.

\subsection{The initial distribution scheme}

\subsubsection*{Charge Distribution}
For any solution triangle $\psi$, the distribution of money is done as follows.

\input{tikz_figures/initial-fractional-charging-scheme-1-2}
\begin{itemize}
    \item If $type(\psi) = 0$, let $f(e) = \frac 1 2$ for any $e \in E(\psi)$. Total distribution is $1.5$ credits.

    \item If $type(\psi) = 3$, let $f(e) = 1$ for any arbitrary edge $e \in E(\psi)$ and $f(e') = 1$ for the edge $e'$ in the $K_4$-subgraph induced by $V(\psi)$ and the anchoring vertex of $\CL_{sin}(\psi)$, such that $e, e'$ do not share any vertex (refer to Proposition~\ref{prop:structures-solution} and Figure~\ref{fig:init-fractional-charging-scheme-1_2}).
    Clearly, we have total distribution of two credits.

    \item If $type(\psi) = 1$, we first define $f(e) =\frac{1}{2}$ for two non-base edges $e$. Then there are two sub-cases.
    \begin{itemize}
        \item  If $\CL_{sin}(\psi) = \{t\}$ and $\psi$ is part of the special structure arising in Proposition~\ref{prop:structures-doubly-attached}, 2. ii), we give $\frac{1}{2}$ each to two non-solution edges of $t$. We refer the base edge of $\psi$ falling in this case as {\em poor base edge} of a type-$1$ triangle.
        Total distribution is two credits in this case.
        \item Otherwise, $|\CL_{sin}(\psi)| \geq 1$, we give $1$ credit to the base edge. We refer the base edge of $\psi$ falling in this case as {\em rich base edge} of a type-$1$ triangle.
        Total distribution is two credits in this case as well.
    \end{itemize}
\end{itemize}

Refer to Figure~\ref{fig:init-fractional-charging-scheme-1_2} for illustration of this scheme.

\iffalse
\begin{itemize}
    \item[type-$0$ triangle:] For each $e \in E(t_0)$, we give them $1/2$ initially. Note that for we still have $1/2$ credit unused for each type-$0$ triangle $t_0$.
    \item[type-$1$ triangle:] We give one to the base edge $e_a$ and $1/2$ to the other green edges.
    \item[type-$3$ triangle:] We want to cover the triangle and all the attached triangles here. Hence, we will pick one green edge and one blue edge and give them one credit each. Note that there are three ways to do this, but all of them are symmetric locally.

\end{itemize}

\fi

For the rest of this section, we are going to assume that all singly-attached triangles of type-$3$ triangles are satisfied, but any doubly-attached or hollow triangle that is adjacent to type-$3$ triangle is always adjacent to a solution edge of the type-$3$ triangle which has no credit.

Following a similar naming convention as for doubly-attached triangles, if $t$ is a hollow triangle adjacent to solution triangles $\psi_1$, $\psi_2$ and $\psi_3$, then $type(t) = [type(\psi_1), type(\psi_2), type(\psi_3)]$ where $type(\psi_1) \leq type(\psi_2)\leq type(\psi_3)$ (see Figure~\ref{fig:hollow-example}).

\input{tikz_figures/hollow_example.tex}

The following proposition captures some structural properties for hollow triangles.

\begin{proposition}[Structures of hollow triangles]
\label{prop:structures-hollow} 
Consider any hollow triangle $t$ adjacent to solution triangles $\psi_1$, $\psi_2$ and $\psi_3$.
\begin{enumerate}
    \item $type(t) \neq [3,3,3]$.
    \item If $type(t) = [1,*,*]$\footnote{If there is no restriction on some dimension, then we put a star ($[*]$) there.} where $type(\psi_1)=1$, then $t$ must be adjacent to the base edge of one of the $\psi_1, \psi_2, \psi_3$ which is a type-$1$ triangle or two type-$1$ triangles from $\{ \psi_1, \psi_2, \psi_3\}$ share a sole anchoring vertex.

    % \item If $type(t) = [1,3,3]$ where $type(\psi_1)=1$, $type(\psi_2)=3$ and $type(\psi_3)=3$, then $t$ must be adjacent to the base edge of $\psi_1$.
    % \item If $type(t) = [1,1,1]$ where $type(\psi_1)=1$, $type(\psi_2)=1$ and $type(\psi_3)=1$, then $t$ must be adjacent to the base edge of at least one of $\psi_1, \psi_2, \psi_3$.
    % \item If $type(t) = [1,1,3]$ where $type(\psi_1)=1$ $type(\psi_2)=1$ and $type(\psi_3)=3$, then $t$ must be adjacent to the base edge of at least one of $\psi_1, \psi_2$.
\end{enumerate}
\end{proposition}


\subsection{Allocating the extra half credit from type-0 triangles}

In the current charge distribution, doubly-attached triangles and hollow triangles which are adjacent to some solution edge having zero credit are not necessarily satisfied. We will transfer the remaining $\frac12$ credits from the type-$0$ triangles to cover these triangles.

Note that the only solution edges which has $0$ credits are either the solution edges of a type-$3$ triangle or a poor base edge of type-$1$ triangle. Whenever these edges participate in doubly-attached triangles and hollow triangles then those triangles might not be covered. But we claim that for any such under-covered doubly-attached or hollow triangle (assuming no benefit comes from type-$3$'s solution edges), there will always be an edge of type-$0$ triangle participating. In particular, this can only happen in type-$[0, 3]$, type-$[0, 1]$, type-$[0, 1, 1]$, type-$[0, 1, 3]$ and type-$[0, 3, 3]$.
In all these cases, we can {\em demand} the $1/2$ remaining credit from that type-$0$ triangle to the common solution edge contained in the type-$0$ triangle to fulfill the non-solution triangles. We call this edge a {\em demanding edge}. Formally, we define every edge of any type-$0$ a demanding edge, if either it is adjacent to any triangle $t \in \tset$ such that $\sum_{e \in E(e)}f(e) < 1$ or it is adjacent to a type-$[0, 3]$ or type-$[0, 3, 3]$ triangle. 
Interestingly, we can prove that for each type-$0$ triangle in $\Nu_0$, there is at most one demanding edge. This ensures that we can assign the remaining $\frac12$ credit for each type-$0$ triangle to its unique demanding edge (if exists) without overcharging (See Fig~\ref{fig:blue-0,3-demanding},\ref{fig:blue-0,1-demanding},\ref{fig:hollow-0,3,3-demanding},\ref{fig:hollow-0,1,3-demanding},\ref{fig:hollow-0,1,1-demanding} for the final charging in various cases)%that is for any type-$0$ triangle, there is at most one solution edge which is adjacent to non-solution triangles which demands the $1/2$ credit from the type-$0$ triangle.

\begin{lemma}[Demand Lemma]
\label{lem:demanding-lemma}
For any triangle $\psi \in \Nu_0$ of type-$0$, there exists at most one demanding edge in $E(\psi)$.
\end{lemma}

The main idea behind the proof for this structural lemma is a local search based argument using the optimality of solution $\Nu$. Whenever there are more than one demanding edge for any type-$0$ triangle, we can use them to find two structures attached to the two demanding edges which allows us to improve the current solution by swapping out some $k$ triangles and adding some other $k+1$ triangles to the solution, contradicting the optimality of $\Nu$.

\iffalse
Hence, some re-distribution scheme is needed. 
We will do this in two phases; \emph{draining phase} and \emph{demanding phase}.

\textbf{Draining re-distribution} For any type-$[1,3]$ doubly-attached triangle $t$, if it falls into Proposition~\ref{prop:structures-doubly-attached}, then let $t_1$ be the type-$1$ triangle adjacent to $t$ and let $t'$ be the attached triangle adjacent to both $t$ and $t_1$. We give $1/2$ credit to edges in $E(t')\setminus E(t_1)$ and remove the credit from $E(t_1) \cap E(t')$. We call the base edge of $t_1$, which now has no credit, \emph{drained} edge (See Fig.~\ref{fig:blue-1,3-draining}).

    \input{tikz_figures/blue-1-3-draining}


\textbf{Demanding re-distribution} After performing draining re-distribution, whenever there is an unsatisfied doubly-attached triangle or hollow triangle $t$ that is adjacent to type-$0$ triangle $t_0$, we will move $1/2$ credit left in $t_0$ to the edge shared between $t$ and $t_0$. This edge will have $1$ credit and we will call this edge \emph{demanding} edge. See Fig~\ref{fig:blue-0,3-demanding},\ref{fig:blue-0,1-demanding},\ref{fig:hollow-0,3,3-demanding},\ref{fig:hollow-0,1,3-demanding},\ref{fig:hollow-0,1,1-demanding} for various cases.

    \input{tikz_figures/blue-0-3-demanding}
    \input{tikz_figures/blue-0-1-demanding}
    \input{tikz_figures/hollow-0-3-3-demanding}
    \input{tikz_figures/hollow-0-1-3-demanding}
    \input{tikz_figures/hollow-0-1-1-demanding}

\begin{observation}
    Even after the re-distributions, all green triangles and attached triangles are still satisfied.
\end{observation}
\fi

    \input{tikz_figures/blue-0-3-demanding}
    \input{tikz_figures/blue-0-1-demanding}
    \input{tikz_figures/hollow-0-3-3-demanding}
    \input{tikz_figures/hollow-0-1-3-demanding}
    \input{tikz_figures/hollow-0-1-1-demanding}

\paragraph{Analysis}
Now we show that all the triangles are satisfied after the demanding allocation. That is, we want to show the following lemma.
\begin{lemma}
   \label{lem:half-main}
    After the demanding allocation step, all the triangles are satisfied and the credits used are at most $2|\Nu|$.
\end{lemma}

It is clear that all the singly-attached and solution triangles are covered.
The demand lemma~\ref{lem:demanding-lemma} tells us that, whenever there is a non-solution triangle $t$, which is adjacent to type-$0$ triangle $\psi_0$, then $t$ is satisfied, i.e., if $t$ is not satisfied, then we make the edge shared between $t$ and $\psi_0$ a demanding edge. Moreover, the bound on the demanding edge from the demand lemma implies that we have enough credits for all the demanding edges.

Now, we take our attention into $\overline{\tset}_0$, the set of non-solution triangles not adjacent to any type-$0$ triangle.

\begin{lemma}
\label{lem:draining-doubly-attached}
    Let $t \in \overline{\tset}_0$ be a doubly-attached triangle then it is adjacent to at most one poor base edge of type-$1$ triangle. Moreover, if $t$ has a poor base edge, then the other solution edge of $t$ is a rich base edge of a type-$1$ triangle.
\end{lemma}

\begin{lemma}
\label{lem:draining-hollow}
    Let $t \in \overline{\tset}_0$ be a hollow triangle then it shares at most two poor base edges with type-$1$ triangles. Moreover,
    \begin{itemize}
        \item  If $t$ has two poor edges, then the third solution edge of $t$ is a rich base edge of a type-$1$ triangle.
        \item If $t$ has one poor base edge of a type-$1$ triangle, then one of the following is true.
        \begin{itemize}
            \item $t$ has at least one rich base edge of some type-$1$ triangle.
            \item $t$ is not adjacent to any type-$3$ triangle.
        \end{itemize}
    \end{itemize}
\end{lemma}

\iffalse
\begin{lemma}
\label{lem:draining-doubly-attached}
    Let $t \in \overline{\tset}_0$ be a doubly-attached triangle then it shares at most one drained edge with type-$1$ triangle. Moreover, if $t$ has a drained edge, then the other green edge of $t$ is a non-drained base edge of a type-$1$ triangle.
\end{lemma}

\begin{lemma}
\label{lem:draining-hollow}
    Let $t \in \overline{\tset}_0$ be a hollow triangle then it shares at most two drained edge with type-$1$ triangle. Moreover,
    \begin{itemize}
        \item  If $t$ has two drained edges, then the third green edge of $t$ is a non-drained base edge of a type-$1$ triangle.
        \item If $t$ has one drained edge, then one of the following is true.
        \begin{itemize}
            \item $t$ has at least one non-drained base edge of some type-$1$ triangle.
            \item $t$ is not adjacent to any type-$3$ triangle.
        \end{itemize}
    \end{itemize}
\end{lemma}

\fi

\paragraph{Proof of Lemma~\ref{lem:half-main}}

%By the way we assign credits, it is clear that we uses at most $2|\Nu|$ credits. 
Assuming Lemma~\ref{lem:demanding-lemma},~\ref{lem:draining-doubly-attached} and~\ref{lem:draining-hollow}; we show that every triangle in $\tset$ is covered.

\begin{enumerate}
    \item All the \cat{solution triangles and singly-attached} triangles are clearly satisfied.
    \item \cat{Doubly-Attached triangles:} There are the following cases.
    \begin{itemize}
      \item \subcat{type-$[0,*]$:}
         In this case, either the triangle already has enough credit or the edge that shared with the type-$0$ triangle becomes a demanding edge.
         Hence, any doubly-attached triangle that shares an edge with type-$0$ triangle is satisfied.
      \item \subcat{type-$[1,1]$:}
         If the triangle has no poor base edge, then it is satisfied.
         Otherwise, by lemma~\ref{lem:draining-doubly-attached}, it is satisfied.
      \item \subcat{type-$[1,3]$:}
         If the edge shared with type-$1$ triangle is a base edge, then it cannot be a poor base edge as it will violate lemma~\ref{lem:draining-doubly-attached}, hence the triangle is satisfied. 
         Otherwise, if it is resulting from Proposition~\ref{prop:structures-doubly-attached}, 2.ii), then it is satisfied by our charging distribution. By Proposition~\ref{prop:structures-doubly-attached}, there cannot be any other case.
      \item \subcat{type-$[3,3]$:}
        By Proposition~\ref{prop:structures-doubly-attached}, such triangles do not exist.
    \end{itemize}
    \item \cat{Hollow triangles:} There are following cases.
    \begin{itemize}
      \item \subcat{type-$[0,*,*]$:} Satisfied by either at least two type-$0$ edges, other type-$1$ edges or the demanding edge of the only type-$0$ triangle.
      \item \subcat{type-$[3, 3, 3]$:} By Proposition~\ref{prop:structures-hollow}, such triangles do not exist.
      \item \subcat{type-$[1,3,3]$:}  If the edge shared with type-$1$ triangle is a base edge, then it cannot be poor-base edge as it will violate lemma~\ref{lem:draining-hollow}, hence the triangle is satisfied. By Proposition~\ref{prop:structures-hollow}, there cannot be any other case.
      \item \subcat{type-$[1,1,*]$:} If it has no poor base edge, then it is satisfied as we have two edges of the type-$1$ triangles with at least half credit each. Otherwise, it is satisfied by lemma~\ref{lem:draining-hollow}.
    \end{itemize}
\end{enumerate}

The total credits used are at most $2|\Nu|$ because (1) the credits are used at most $2|\Nu|$ initially and (2) the credit used for demanding edges are charged to the extra $\frac12$ credits remaining with type-$0$ triangles. Moreover, by Lemma~\ref{lem:demanding-lemma}, each type-$0$ triangle will get charged at most once, hence the total credits bound follows.

This complete the proof for Lemma~\ref{lem:half-main}.

==> tex/type-1_3.tex <==

\section{Transversal for type-$1$\&$3$ instances}
\label{sec:type-13-transversal}
In this section, we assume that there are no type-$0$ triangles in our solution $\Nu$. We will show that for these instances $\tau(G) \leq (2 + \frac13) \nu$. This is equivalence to finding the assignment $f: E \rightarrow {\mathbb R}^+$ such that $f(e) \in \{0, 1\}$ where $\sum_e f(e) \leq (2+\frac13) |\Nu|$ and for all $t \in \tset$, $\sum_{e \in E(t)} f(e) \geq 1$.


%\subsection{The initial distribution scheme}
%\begin{figure}[H]
%    \centering
%    %\includegraphics{}
%    \caption{Initial Integral Traversal Charging}
%    \label{fig:initial-2.33}
%\end{figure}


\paragraph{Generalized-Pair-Structure} Here we extend the notion of $PAIRS \subseteq \Nu_1 \times \Nu_1$. Recall that we constructed a set $PAIRS \subseteq \Nu_1 \times \Nu_1$ to contain all pairs $\{\psi_1, \psi_2\}$ of type-$1$ solution triangles such that there is a non-solution triangle $t$ doubly-attached to $\psi_1$ and $\psi_2$ and $\{\psi_1, \psi_2\}$ forms a pair in the sense of Proposition~\ref{prop:type-[1-1]}.\ref{itm:pair}.


The triangle $t$ is called the \textit{defining triangle} for the pair.

Now we construct another set $PAIRS' \subseteq \Nu_1 \times \Nu_1$ to contain all pairs $\{\psi_1, \psi_2\}$ of type-$1$ solution triangles such that there is a non-solution type-$[1,1,3]$ hollow triangle $t$ adjacent to $\psi_1$ and $\psi_2$ and $\{\psi_1, \psi_2\}$ share their anchoring vertex.
\begin{figure}[H]
    \centering
    %\includegraphics{}
    \caption{Generalized Stem structure}
    \label{fig:GenStemStructure}
\end{figure}

For each pair $\Psi = (\psi_1, \psi_2) \in PAIRS'$, we again use $anchor(\Psi)$ to denote the common anchor between $\psi_1$ and $\psi_2$ and $cv(\Psi)$ to denote the common vertex in $V(\psi_1) \cap V(\psi_2)$ and {\em stem} of the pair $\Psi$ to refer to the (non-solution) edge that connects $cv(\Psi)$ to $anchor(\Psi)$.
Let $\mathcal{P} := \bigcup_{(\psi, \psi') \in PAIR\cup PAIR'} \{\psi, \psi'\}$.

% \begin{lemma}[Generalized Stem Lemma]
% \label{lem:generalized-stem}
% Let $\psi$ be a solution triangle and $\nset(\psi) := \{\psi': \{\psi, \psi'\} \in PAIRS \cup PAIRS' \}$ be the set of all other solution triangles $\psi'$ that form a pair with $\psi$.
% Then, we have that for any $\psi_1, \psi_2 \in \nset(\psi)$, we have $stem(\psi, \psi_1) = stem(\psi, \psi_2)$.
% \end{lemma}

\paragraph{Flower-Structure} Now we define a {\em flower} structure. The {\em core} $\psi \in \Nu_3$ of the flower structure will be a type-$3$ triangle. The {\em petals} $\{\psi_1, \psi_2\} \in \Nu_1 \times \Nu_1$ will be a part of the structure iff 1) there exists a type-$[1,1,3]$ hollow triangle $t$ adjacent to $\psi, \psi_1, \psi_2$ and 2) $anchor(\psi) = anchor(\psi_1) = anchor(\psi_2)$.

\begin{figure}[H]
    \centering
    %\includegraphics{}
    \caption{Flower Structure}
    \label{fig:FlowerStructure}
\end{figure}

\subsubsection*{Lending Relations}
    Here, let us define two relations that will be used afterward in the charge distribution and in the analysis.
    
    \begin{definition}
        Let $lend \subseteq \Nu_1 \times \Nu$ be a relation (possibly $\empty$) from type-$1$ triangles $\Nu_1$ to solution triangles $\Nu$.
        % When $(t, t') \in lend$, it means that we might give away a credit of $t$ to for the usage of $t'$.
    If there exists a doubly attached triangle $t$ adjacent to triangles $\psi_1 \in \Nu_1$ and $\psi \in \Nu$ such that $|\CL_{sin}(\psi_1)| = 1$ where the only anchoring vertex is in $V(\psi)$; in this case, $(\psi_1, \psi) \in lend$ (see Fig.~\ref{fig:lend-structure}). In addition, we also define a function $gain_1 \colon lend \rightarrow E \cup \varnothing$, where $gain_1((\psi_1, \psi)) := E(t) \cap E(\psi)$.
    
    We want $lend$ relation to be anti-symmetric, in the other word, if both $(\psi, \psi')$ and $(\psi', \psi)$ can be in $lend'$, then we will select only one of these two arbitrarily.
    
    \end{definition}
    \begin{definition}
        Let $lend' \subseteq \Nu_1 \times \Nu_3$ be a function that points from a triangle $\psi \in \Nu_1$ to another triangle $\psi' \in \Nu_3$. This can be empty.
        
        We say that $(\psi_1, \psi) \in lend'$ if there exists a triangle $\psi_2$ such that $\{\psi_1, \psi_2\}$ is a petal of a flower which $\psi$ is a core.
        
        We define $gain_2 \colon lend' \rightarrow E \cup \varnothing$ as follows. For each $(\psi_1, \psi) \in lend'$, there exists a type-$[1,1,3]$ triangle $t$ that adjacent to $(\psi_1, \psi_2, \psi)$, we let $gain_2( (\psi_1, \psi) ) := E(t) \cap E(\psi)$.
        % When $(t, t') \in lend'$, it means that we might give away a credit of $t$ to for the usage of $t'$. 
    \end{definition}
    
    The following structural lemma will be useful to define a valid charging.
   
\paragraph{Directed Pseudoforest graph} Using solution triangles $\Nu$ as the vertex set and ordered pairs $A = lend \cup lend'$ as edge set, we define the digraph $\Gamma = (\Nu, A)$. For clarity, we will refer to the vertices $\Nu$ as {\em nodes} and edges $A$ as {\em arcs} to differentiate from vertices/edges of $G$.

\begin{lemma}
\label{lem:gen-outdegree} For any $\psi_1 \in \Nu_1$, the out-degree  $d^+_\Gamma(\psi_1)$ is at most one and for any $\psi_3 \in \Nu_3$, the out-degree $d^+_\Gamma(\psi_3)$ is zero.
\end{lemma}\sumi{This holds!}
\begin{proof}
The second property of $d^+_\Gamma(\psi_3) = 0$ is true by the way we define the relations $lend$ and $lend'$.

Let there be a solution triangle $\psi \in \Nu_1$ such that $d^+_\Gamma(\psi) \geq 2$. Let $\psi_1$ and $\psi_2$ be the solution triangles corresponding to the out-neighbours of $\psi$. 
\end{proof}

The lemma above implies that $\Gamma$ is a directed pseudoforest\footnote{See \url{https://en.wikipedia.org/wiki/Pseudoforest\#Directed_pseudoforests} for definition}. 

Now for simplicity, we define a combine function $gain \colon \Nu \rightarrow E \cup \varnothing$. We say that $gain(\psi) := e$ if there exists $\psi_1$ such that $gain_1((\psi, \psi_1)) = e$ or $gain_2((\psi, \psi_2)) = e$ otherwise $gain(\psi) = \varnothing$. Notice that $gain$ is a well defined function as any node $\psi$ has out-degree $d_\Gamma^+(\psi) <= 1$ hence there will be a unique $e$ (if exists).

\begin{observation}
\label{obs:pseudo-properties}
    The following properties hold for any connected component $C$ of $\Gamma$:
    \begin{itemize}
        \item There can be at most one cycle in $C$.
        \item If there is a cycle in $S$, then every node in $V(S)$ corresponds to a type-$1$ triangle. Moreover, all the arcs (if exists) incident to the cycle will be directed towards the cycle. Also, all nodes in $V(C)$ corresponds to type-$1$ triangles.
        \item If $C$ does not have cycle, then $C$ must be anti-arborescence. Every non-root node must correspond to a type-$1$ triangle. The root can be either type-$1$ or type-$3$ triangle.
        % \item In $C$, if there is a vertex $v \in V(C)$ corresponding to type-$3$ triangle, then it must be the root of anti-arborescence $C$, i.e., $C$ must not have any cycle.
    \end{itemize}
\end{observation}

The following lemma tells us about out degree of nodes corresponding to pairs. 

\begin{lemma}
\label{lem:pair-zero-degree}
For any triangle $\psi \in \mathcal{P}$, the out-degree $d^+_\Gamma (\psi)$ is zero.
\end{lemma}\sumi{NOT TRUE!}
\paragraph{Charge Distribution}
Now we are ready to start distributing the $2 |\Nu|$ credits from triangles in $\Nu$ to edges in $E$ by modifying function $f$. In process, we will use $\Gamma$ to lend some credits across triangles in $\Nu$.
We start with $f(e) = 0 \, \, \forall e \in E$.

\paragraph{Charge lending using $\Gamma$}
Now we iterate over the components of $\Gamma$ independently to lend charge across triangles in $\Nu$. 
We will first define a set of arcs to be \emph{active} and then decide where to transfer credits based on these active arcs.
For any acyclic component $C$ of $\Gamma$, the $root$ of $C$ is a vertex such that $d^+_\Gamma(root) = 0$. We work in a top-down fashion starting from $root$, i.e., we decide first whether the arcs in $\delta_\Gamma^-(root)$ are active. If $C$ has a cycle $S$, then we begin from $S$ by treating it as a super root. We then work(re-curse) on the its children.
\begin{enumerate}
    \item If $C$ has a cycle $S$, then we mark every arc $a$ of $E_\Gamma(S)$ to be active. Then for any $\psi \in V_\Gamma(S)$, we select another incoming arc $a'$ to be active. If $\psi$ has $d_\Gamma^-(\psi) > 1$, then the choice can be made arbitrarily.
    \item Otherwise, let $r$ be the current node (which is the $root$ at the beginning of the procedure).
    \begin{enumerate}
        \item If it does not have any incoming arc, i.e., if $d_\Gamma^-(r) = 0$, then we don't have to do anything.
    \item If $d_\Gamma^+(r) = 0$ or the edge in $\delta_\Gamma^+(r)$ is not active, then we select any one incoming arc in $\delta_\Gamma^-(r)$ to be active.
        \item If the arc $\delta_\Gamma^+(r)$ is active then we select up to two incoming arcs in $\delta_\Gamma^-(r)$ to be active.
    \end{enumerate}
    \item Repeat step 2. iteratively for the children $N^-_\Gamma(r)$ of the current node $r$ (or $N^-_\Gamma(C)$ of the current cycle $C$).
\end{enumerate}

Let $A^+$ be set of all the active arcs. Now we assign $f$ as follows.
\begin{enumerate}
    \item If $\psi$ has more active incoming arc(s) than active outgoing arc, then we assign $f(e) = 1$ for every edge $e \in E(\psi)$.
    \item Otherwise If $\psi \in \Nu_3$, then we look at the $K_4$ consisting of vertices $V(\psi) \cup anchor(\psi)$ and pick two edges $e, e'$ that do not share any end point. We set $f(e) = 1$ and $f(e') = 1$.
    \item Otherwise If $\psi \in \Nu_1$, if $\psi$ has an active incoming arc and an active outgoing arc. We set $f(gain(\psi)) = 1$ and $f(base(\psi)) = 1$.
    \item If $\psi \in \Nu_1$ and if $\psi$ has an active outgoing arc but no active incoming arc, then we only set $f(base(\psi))=1$.
    \item Otherwise, if $\psi \in \mathcal{P}$, then we set $f(base(\psi)) = 1$ and $f(e) = 1$ where $e \in E(\psi)$ is the non-base edge of $\psi$ adjacent to its stem. 
   \item If $\psi \in \Nu_1 \setminus \mathcal{P}$ and does not have any incoming or outgoing active arc, then we set $f(base(\psi)) = 1$ and we reserve its extra $1$ credit for later use.
\end{enumerate}

The proposition below implies that we do not overcharge triangle in $\Nu$.

\begin{proposition}
\label{prop:lend-distribution}
For any non-singleton component $C$ of $\Gamma^+ = (\Nu, A^+)$, $\sum_{e \in E_{\Gamma^+}(C)} f(e) = 2 |V_{\Gamma^+}(C)|$.
\end{proposition}

 

The following lemma is true for the current credit distribution function $f$.


\begin{lemma}
\label{lem:partial-cover}
    For any triangle $t$ of graph $G$, if $\sum_{e \in E(t)} f(e) = 0$, $t$ is a type-$[1,1,1]$ hollow triangles.
\end{lemma}

Let the set of type-$[1, 1, 1]$ triangles which are not covered be $\mathcal{H}$.

\paragraph{Friends triangles} 
Now we define {\em friends} triangles based on the following lemma.

\begin{lemma}[Friends Lemma]
\label{lem:friends} For any type-$[1, 1, 1]$ hollow triangle $t \in \mathcal{H}$ adjacent to $\{\psi_1, \psi_2, \psi_3\}$, there exists exactly two type-$1$ triangles $\psi, \psi' \in \{\psi_1, \psi_2, \psi_3\}$, such that $anchor(\psi) = anchor(\psi')$.
\end{lemma}

We define any two type-$1$ triangles $\{\psi, \psi'\}$ coming from the Friends Lemma as {\em friends}. Let $\mathcal{F}$ be the set containing all these triangles.

The following claim holds.

\begin{claim}
\label{clm:pairs-friends-disjoint}
$\mathcal{P} \cap \mathcal{F} = \emptyset$.
\end{claim}

\begin{lemma}
\label{lem:friends-zero-degree}
For any triangle $\psi \in \mathcal{F}$, the out-degree $d^+_\Gamma (\psi)$ is zero. Moreover, there is no incoming active arc incident on $\psi$ and $f(e) = 0$ for any $e \in E[\psi] - base(\psi)$.
\end{lemma}

The above lemma implies that for each $\psi \in \mathcal{F}$, $\psi$ has a reserved credit. Let us define $NB_{\mathcal{F}} := E[F] \setminus base[F]$ as the set of non-base edges of triangles in $\mathcal{F}$.

Now for any type-$1$ triangle $\psi \in \Nu_1 \setminus (\mathcal{F} \cup \mathcal{P})$ which still has a reserved credit, pick any arbitrary edge $e \in E(\psi)$ such that $f(e)=0$ and assign $f(e) = 1$. It is clear, that $e$ will be some non-base edge.

Now let $P = \{e : e \in E(\psi) \wedge f(e) = 0 \wedge \psi \in \Nu \setminus \mathcal{F} \}$.
After the last step, the following lemma holds.
\begin{lemma}
\label{lem:poor-non-base} \[|P| \leq |\Nu \setminus \mathcal{F}|\]
\end{lemma}

The Lemma~\ref{lem:friends} and~\ref{lem:poor-non-base} above implies the following observation.

\begin{observation}
Each triangle in $t \in \mathcal{H}$ is adjacent to only non-base edges of $\mathcal{F}$ and edges in $P$. Moreover, each triangle $t$ has at least two non-base edge of $\mathcal{F}$.
\end{observation}

Using the observation above, we can cover the triangles in $\mathcal{H}$ in the following two ways and take the one which minimized $\sum_{e \in E} f(e)$.
\begin{enumerate}
    \item (\textbf{Bi-partization}) We know that graph $G' = (V, P \cup NB_{\mathcal{F}})$ can be made bipartite by removing an edge set $E'\subseteq P \cup NB_{\mathcal{F}}$ such that $|E'| \leq |P \cup NB_{\mathcal{F}}|/2$. We assign $f(e) = 1 \,\, \forall e \in E'$.
    \item Assign $f(e) = 1 \,\, \forall e \in NB_{\mathcal{F}}$.
\end{enumerate}

\begin{theorem}
\label{thm:factor-2.33}
It holds that $\sum_e f(e) \leq (2+\frac13) |\Nu|$ and for all $t \in \tset$, $\sum_{e \in E(t)} f(e) \geq 1$.
\end{theorem}

\begin{proof}
    We first show that every triangle is covered, i.e., $\sum_{e \in E(t)} f(e) \geq 1$ for any triangle $t$.
    By Lemma~\ref{lem:partial-cover} and Lemma~\ref{lem:friends}, after we distribute the lending charges, the only triangles not covered are triangles in $\mathcal H$. Those triangles are surely be covered by our final charging, hence every triangle must be covered.
    
    Now, notice that the credits used would be the minimum one between 
    $2|\Nu| - |\mathcal F| + (2|\mathcal F| + |P|) / 2 \leq 2|\Nu| - |\mathcal F| + (|\Nu| + |\mathcal F|)/2 = 2.5|\Nu| - |\mathcal F|/2 $ (bi-partization) and
    $2|\Nu| - |\mathcal F| + (2|\mathcal F|) = 2|\Nu| + |\mathcal F|$.
    
    The minimum between the two would be maximized if these two terms hold the same value, in the other word when
    \begin{align*}
        2.5|\Nu| - |\mathcal F|/2 &= 2|\Nu| + |\mathcal F| \\
        |\Nu| &= 3|\mathcal F|.
    \end{align*}
    
    Once we substitute this equality back, we get that $\sum_e f(e) \leq (2 + \frac{1}{3})|\Nu|$.
    
    

\end{proof}


==> tikz_figures/demand-two-doubly-attached-one-type-3-one-type-1-common-t_rr.tex <==
\begin{figure}[ht]
            \centering
            %\includegraphics[width=0.3\textwidth]{figures/demand-two-doubly-attached-one-type-3-one-type-1-common-t_rr.png}
        \subfloat{
        \begin{tikzpicture}[scale=0.6, every node/.style={scale=0.8}]
        \draw [fill=lightgray] (0,0) -- (1.5,2) -- (3,0) -- (0,0);
        \draw [fill=lightgray]  (3,0) -- (6,0) -- (4.5,2) -- (3,0);
        \draw [line width=2pt, fill=lightgray] (1.5,2) to [out=30,in=180] (5,3) to [out=0,in=100] (6,0) to (6.75,4) to [out=40,in=195] (1.5,2);
        \GraphInit[vstyle=Normal]
\tikzset{VertexStyle/.style = {shape=circle, fill=white, draw=black, inner sep=1pt, minimum size=20pt}}
        \Vertex{a}
        \Vertex[y=2,x=1.5]{b}
        \Vertex[y=0,x=3]{c}
        \Vertex[y=2,x=4.5]{d}
        \Vertex[y=0,x=6]{e}
        \Vertex[y=4,x=6.75]{f}
        \SetUpEdge[
            lw = 2pt,
            color = black,
        ]
        \Edges(a,b,c,a)
        \Edges(c,d,e,c)
        %\tikzstyle{EdgeStyle}=[bend left=20]
        %\Edge(b)(f)
        %\tikzstyle{EdgeStyle}=[out=20,in=110]
        %\Edge(b)(e)
        \SetUpEdge[
            lw = 1pt,
            color = black,
            style = dashed
        ]
        \Edge(b)(d)
        \Edge(d)(f)
        \tikzstyle{EdgeStyle}=[bend right=15]
        \Edge(c)(f)
        \tikzstyle{EdgeStyle}=[bend right=25]
        \Edge(a)(e)
        \end{tikzpicture}
        }
            \caption{$t_0=\Delta^0_{abc}$ is type-$0$, $t_{\ell\ell}=t_{r3}= \Delta^3_{bef}$ is type-$3$ and $t_{rr}=\Delta^1_{cde}$ is type-$1$. $\Delta^3_{abc}$ is a common type-$3$ triangle responsible for making the base edge of $\Delta^1_{cde}$ poor and forms the doubly-attached type-$[0, 3]$ triangle $t_\ell=\Delta_{bea}$ in this configuration with a common vertex with $\Delta^1_{cde}$. The other doubly-attached triangle is $t_r = \Delta_{bcd}$. \textbf{Impossible because there is an improving $3$-swap.}}
            \label{fig:demand-two-doubly-attached-one-type-3-one-type-1-common-t_rr}
         \end{figure}

